Truncation in Differential Hahn Fields

Being closed under truncation for subsets of generalized series fields is a robust property in the sense that it is preserved under various algebraic and transcendental extension procedures. Nevertheless, in Chapter 4 of this dissertation, we show that generalized series fields with truncation as an extra primitive yields undecidability in several settings. Our main results, however, concern the robustness of being truncation closed in generalized series fields equipped with a derivation, and under extension procedures that involve this derivation. In the last chapter, we study this in the ambient field $\mathbb{T}$ of logarithmic-exponential transseries. It leads there to a theorem saying that under a natural `splitting' condition the Liouville closure of a truncation closed differential subfield of $\mathbb{T}$ is again truncation closed.

==> ConstantskkfM.tex <==
As in Section \ref{extderco} and Lemma 6.1 Which I would add a label and a reference to later we have
\begin{lemma} The following conditions are equivalent: \begin{enumerate}
\item[\rm{(i)}] for every $n$ the map $c_n: \fM_n\to \smallk_{n-1}$ is injective and $c_n(\fM_n)\cap \smallk_{n-1}^\dagger=\{0\}$;
\item[\rm{(ii)}] $\smallk[[\fM]]$ has the same constant field as $\smallk$.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $f\in \smallk[[\fM]]$. Let $\fm=\fm_0\cdots \fm_n\asymp f$ with $n = \min\{k: \fm \in \fM^{(k)}\}$. We now assume that $n\neq -1$ and consider that case later. We let 
\[f_\fm := \sum_{\substack{\fn\in \fM^(n-1)\\ \fn\fm_n \in \supp(f)}} f_{\fn\fm_n}\fn.\]
We then have 
\[\der(f) = (\der(f_\fm) +f_\fm c_n(\fm))\fm + (\text{ terms } \prec_\fM^{(n)} \fm).\] 
Thus if (i) holds, then $f\asymp_{\fM} \der(f)$. If $F\asymp 1$, then $\der(f) = \der(f-f_1) + \der(f_1)$. By the argument above, the only way that $\der(f)$ is zero in this case is if $f-f_1 = 0$, and $\der(f_1) = 0$, concluding the proof that (i) implies (ii). Now, if $c:\fM \rightarrow \smallk[[\fM]]$ is not injective, then there is $\fm\in \fM$ such that $\der(\fm) = c(\fm)\fm = 0$. On the other hand, assume that $A:=c_n(fM_n)\cap (\smallk_{n-1}^*)^\dagger\neq \{0\}$. Let $cn(\fm) = f^\dagger\in A$ for some $\fm \in \fM_n$ and $f\in \smallk_{n-1}^*$. Then $\der (f\fm)= 0$, proving (ii) implies (i). 
\end{proof}

==> NIP.tex <==
\section{NIP}

As is customary in Model Theory, certain theories are classified by having a lack of a certain ``bad'' property. A clear example, and focus of this section is the \textbf{independence property}. Given an $L$-theory $T$, we say that a partitioned $L$-formula $\phi(x;y)$ has the independence property if there is a model $M$ of $T$ and an infinite subset $X$ of $M^{x}$  that is \textbf{shattered} by $\phi$, i.e. for any $A\subseteq X$ there is $b_A\in M^y$ such that for $X\cap \phi(x;b_A)= A$. By compactness this is equivalent to saying that there is a model $M$ of $T$ such that for every $n$, the formula $\phi(x;y)$ shatters a subset of $M^x$ of size $n$.  
\begin{example} Let $T$ be the theory of Peano Arithmetic, then the formula $\phi(x;y) = \exists z (xz=y)$ has the independence property. Indeed, let $P$ be the set of primes, $A\subseteq P$, and $b_A = \prod_{p\in A} p$. Then $\phi(x;b_A)\cap P = A$.
\end{example}

\begin{lemma} A formula $\phi(x;y)$ has IP if and only if there is an indiscernible sequence $(a_n)_n$ and a tuple $b$ such that $\phi(a_n;b)$ holds if and only if $n$ is even. 
\end{lemma}
\begin{lemma} A formula $\phi(x;y)$ is NIP if and only if for any indiscernible sequence $(a_n)_{n}$ and any parameter $b$ the formula $\phi(a_n,b)$ eventually holds or is eventually false.
\end{lemma}


\noindent
Note that if the formula $\phi(x;y,d)$ has IP, where $d$ is a $|z|$-tuple of parameters, then the formula $\phi(x;yz)$ has IP.
A formula is said to be \textbf{NIP} if it does not have the independence property. 
A theory $T$ is said to be NIP if no formula has the independence property. 
\begin{example} The theory of dense linear orders with no endpoints is NIP. Indeed, by quantifier elimination and \ref{boolNIP} it is enough to check the formulas $x<y$ and $x=y$.
\end{example}
